A Decade of Information Architecture in HCI: A Systematic Literature Review

Information Architecture (IA) is a blueprint for the information system in websites or other information-rich environments. It corresponds to how we organize, label and structure information. The importance of Information Architecture and its influence on a system's usability is vastly discussed in literature. Because of the inherent connection between Information Architecture concepts and the Human Computer Interaction (HCI) field, we decided to investigate how previous research has used Information Architecture in the context of Human Computer Interaction (IAinHCI). In order to do that, we followed a two phase process. First, we conducted a Systematic Literature Review (SLR). We queried both the ACM and IEEE databases. We filtered and assessed 311 papers that spanned a decade of research on Information Architecture. We found 25 papers that utilized Information Architecture in the context of Human Computer Interaction. Then, we followed a Background Reference Search process using the SLR resulting papers as a starting set. We assessed the eligibility of the reference list of all 25 papers and found eight additional papers that were relevant to our research question. Results of our review show that, IAinHCI papers fall under seven main categories, from IoT to the semantic web and ubiquitous technology. The website category, however, was both the most consistent over the years and the most prevalent category accounting for 67% of the papers. Our findings suggest that IA has not yet uncovered its full potential and there is still room for research to leverage and expend the IA knowledge base promising a prosperous future for Information Architecture.

==> tables/SLRpapers.tex <==
\begin{table*}[bht!]
  \begin{tabular}{L{0.5cm}L{8.3cm}L{8.1cm}}
%  \begin{tabular}{L{2.5cm}C{1.5cm}L{6.25cm}L{10cm}}
  \hline
     {\small \textbf{ } }
%    & \small \textbf{ } }
    & {\small \textbf{Websites}} 
    & {\small \textbf{Papers}}  
    \\\hline
%%%%% NEW ROW. %%%%%
    \multirow{4}{*}{
    {\rotatebox{90}{\parbox{1.1cm}  {\centering\small Design /Eval}}}}
%   &  \small }
    & \small Collaborative Websites
    & \small Paper ref
    \\\cline{2-3}
   
%  & \small } 
  & \small Non collaborative websites (visual IA)
  & \small paper ref \\\cline{2-3}

%  & \small } 
  & \small Non collaborative websites (Aural IA)
  & \small paper ref \\\cline{2-3}
  
%  & \small } 
  & \small Educational: Online education/ OER/ Academic websites
  & \small paper ref \\ \hline
\multirow{2}{*}{
    {\rotatebox{90}{\parbox{1.1cm}  {\centering\small Design /Eval}}}}
    %   &  \small }
    & \small Collaborative Websites
    & \small Paper ref
    \\\cline{2-3}
   
%  & \small } 
  & \small Non collaborative websites (visual IA)
  & \small paper ref \\\hline
%%%%% NEW ROW. %%%%%
 {\small \textbf{ } }
%    & \small \textbf{ } }
    & {\small \textbf{Mobile Apps}} 
    & {\small \textbf{Papers}}  
    \\\hline
 \multirow{2}{*}{
    \rotatebox{90}{\parbox{1.7cm}  {\centering\small Design/ Eval}}}%: Contribute to the documentation}}}
% &  \small  }
 &  \small \textit Visual IA 
 & \small ref
 \\ \cline{2-3}
%  &  \small }
  &   \small Aural IA
  &  \small ref
  \\ \hline

%%%%% NEW ROW. %%%%%
 \multirow{2}{*}[0.7em]{
    \rotatebox{90}{\parbox{1.7cm}  {\centering\small F7-FileIssue}}}%: File an Issue [in the issue tracker]} }}
% &  \small }
 &  \small \textit{Issue 5:} ``...nothing clearly says that filing an issue is part of contributions. No clear instruction about what she needs to do... it doesn't say where to find the issue list'' \newline \textit{Facets: SE, Risk, Info}
 &  \small Added hint in \texttt{README.md} about filing an issue \textit{(Labeling-Keyword)}, added instructions \textit{(OrgScheme-Task)} with link to the ``Issue list'' \textit{(Nav-Link)}. Figure in supplemental document.\\ \cline{2-3}
% &  \small  }
 &  \small \textit{Issue 6:} ``[referring to the Issue Form] she may not know what to put in, no steps of what to include'' \newline \textit{Facets: Risk, Info}
 &  \small Created an issue template\textit{(Org Scheme-Task)}. \newline Shown in Figure~\ref{fig:Issue_template}. \\ \hline

%%%%% NEW ROW. %%%%%
 \multirow{2}{*}{
    \rotatebox{90}{\parbox{1.7cm}  {\centering\small U2-Setup}}}%:\\ Set up the environment}}}
% & \small   }
 & \small \textit{Issue 7:} ``...nothing that explicitly says set up the env...She would read through step 0 and think it's not for mac [OS] and not know what to do...'' \newline \textit{Facets: SE, Risk, Info}
 & \small Added hint in \texttt{README.md}
 that guides to the right details about setting up the environment \textit{(Labeling-Keyword)}, reorganized parts of \texttt{contributing.md} \textit{(OrgStruct, OrgScheme-Topic)} and added links \textit{(Nav-Link)}. Figure in supplemental document.
 \\ \cline{2-3}

% & \small   }
 & \small \textit{Issue 8:} ``%Not enough information on each step and why it's there. 
 ...No explanation about the different things to install and where to install them''. \newline \textit{Facets: Motiv, SE, Risk, Info, Learn}
 & \small Added hint in a sub-page of \texttt{contributing.md} about executing commands \textit{(Labeling-Keyword)} and added additional explanation about each command. Shown in Figure~\ref{fig:BeforeAfterEnv}.
 \\ \hline
   
  \end{tabular}
  \caption{For each Study~\#2 use-case, the issues and fixes associated with Project~F's IA elements. Issues excerpted from Team~F's analysis forms. 
  }
 \label{table:FlossIssuesFixes}
 \vspace{-5mm}
\end{table*}

==> tables/results.tex <==
\begin{table}[b!]
% \scriptsize
\begin{tabular}{L{1.9cm}L{6.5cm}L{1cm}}
%\hline
    { \scriptsize \textbf{Cat}}
    & { \scriptsize \textbf{Descriptions}}
    & { \scriptsize \textbf{Teams}}
    \\\hline

%\hangindent=1em
%\hangafter=1
    \scriptsize  U1-Familiarize
    & \scriptsize Familiarize with the project \& find a task to work on
    & \scriptsize C\\%\hline

%\hangindent=1em
%\hangafter=1
     \scriptsize U2-Setup
     & \scriptsize Set up the environment
     & \scriptsize A,~C,~E,~F
    \\%\hline

%\hangindent=1em
%\hangafter=1
     \scriptsize U3-Find
     & \scriptsize Use GitHub issue tracker to find a task
     & \scriptsize B, D, F
    \\%\hline

%\hangindent=1em
%\hangafter=1
     \scriptsize U4-PullHelp
     & \scriptsize Find help on how to do a pull request
     & \scriptsize B, D
    \\%\hline

%\hangindent=1em
%\hangafter=1
     \scriptsize U5-Review
     & \scriptsize Review a previously submitted pull request 
     & \scriptsize B
    \\%\hline

%\hangindent=1em
%\hangafter=1
     \scriptsize F6-Document
     & \scriptsize Contribute to the documentation 
     & \scriptsize F
    \\%\hline

%\hangindent=1em
%\hangafter=1
     \scriptsize F7-FileIssue
     & \scriptsize File an issue in the Issue Tracker
     & \scriptsize F
    \\\hline

    
\end{tabular}
\caption{The use-cases in the two studies. The first five were chosen because they have previously been shown to pose barriers to OSS newcomers~\cite{Steinmacher-2015-(CSCW),sarma2016FSE}. The last two were chosen because they were particularly important to Team~F (Study~\#2).}
\label{table:usecasesdescriptions}

\vspace{-4mm}
\end{table}
